LUX-ZEPLIN (LZ) Technical Design Report

In this Technical Design Report (TDR) we describe the LZ detector to be built at the Sanford Underground Research Facility (SURF). The LZ dark matter experiment is designed to achieve sensitivity to a WIMP-nucleon spin-independent cross section of three times ten to the negative forty-eighth square centimeters.

==> LZtdrSupport/LZsym.tex <==
%%%%%   Symbols for use in LZ
%%%%%
%%%%%   Revised from BaBar/SuperB/accelerator to LZ  08/17/2015  H. Nelson
%%%%%

\RequirePackage{xspace}

\RequirePackage{hyperref}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\mathrm{t}}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\mathrm{t}}$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\mathrm{ES}}$}\xspace}
\def\mec        {\mbox{$m_{\mathrm{EC}}$}\xspace}
\def\DeltaE     {\mbox{$\Delta E$}\xspace}

\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\keVee}{\si{\keV\ee}}
%\newcommand{\keVnr}{\si{\keV\nr}}
%\newcommand{\keVvis}{\si{\keV\vis}}
\DeclareRobustCommand{\Pga}{\HepParticle{\alpha}{}{}\xspace} % alpha
\DeclareRobustCommand{\Pgb}{\HepParticle{\beta}{}{}\xspace} % beta
\DeclareRobustCommand{\Pgd}{\HepParticle{\delta}{}{}\xspace} % delta
\DeclareRobustCommand{\Pgbm}{\HepParticle{\beta}{}{-}\xspace} % negative beta
\DeclareRobustCommand{\Pgbp}{\HepParticle{\beta}{}{+}\xspace} % positvie beta
\DeclareRobustCommand{\Pd}{\HepParticle{d}{}{}\xspace} % deuteron
\DeclareRobustCommand{\Pad}{\HepAntiParticle{d}{}{}\xspace} % anti-deuteron
%\newcommand{\perkkd}{\si{\per\keV\per\kg\per\day}} % /keV/kg/day
%\newcommand{\perkgd}{\si{\per\keV\per\day}} % /kg/day
%\newcommand{\perktd}{\si{\per\keV\per\tonne\per\day}} % /keV/tonne/day
%\newcommand{\pertd}{\si{\per\tonne\per\day}} % /tonne/day
%\newcommand{\perkty}{\si{\per\keV\per\tonne\per\year}} % /keV/tonne/year
%\newcommand{\perty}{\si{\per\tonne\per\year}} % /tonne/year

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\,\mathrfm{in}}\xspace} % \in is taken
\def\ft   {\ensuremath{\,\mathrfm{ft}}\xspace}
\def\km   {\ensuremath{{\,\mathrm{km}}}\xspace}
\def\m    {\ensuremath{{\,\mathrm{m}}}\xspace}
\def\msquare {\ensuremath{{\,\mathrm{m}}^2}\xspace}
\def\cm   {\ensuremath{{\,\mathrm{cm}}}\xspace}
\def\cma  {\ensuremath{{\,\mathrm{cm}}^2}\xspace}
\def\cubicm   {\ensuremath{{\,\mathrm{m}}^3}\xspace}
\def\mm   {\ensuremath{{\,\mathrm{mm}}}\xspace}
\def\mma  {\ensuremath{{\,\mathrm{mm}}^2}\xspace}
\def\mum  {\ensuremath{{\,\mu\mathrm{m}}}\xspace}%% mu meter
\def\muma {\ensuremath{{\,\mu\mathrm{m}}^2}\xspace}
\def\nm   {\ensuremath{{\,\mathrm{nm}}}\xspace}
\def\fm   {\ensuremath{{\,\mathrm{fm}}}\xspace}
\def\nm   {\ensuremath{{\,\mathrm{nm}}}\xspace}   %% nanometer
%
% integrated cross section, exposure
\def\barn{\ensuremath{{\,\mathrm{b}}}\xspace}
\def\barnhyph{\ensuremath{{\mathrm{-b}}}\xspace}
\def\mbarn{\ensuremath{{\,\mathrm{mb}}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb{\ensuremath{{\,\mathrm{nb}}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\,\mathrm{pb}}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\ab   {\ensuremath{\mbox{\,ab}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}
\def\designlumi {\ensuremath{10^{36}\cms}\xspace}
\def\lumi {\cms\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\,\mus}\xspace}
\def\ns   {\ensuremath{\,\mathrm{ns}}\xspace}
\def\ps   {\ensuremath{\,\mathrm{ps}}\xspace}
\def\fs   {\ensuremath{\,\mathrm{fs}}\xspace}

%Mass
\def\gm   {\ensuremath{\,\mathrm{g}}\xspace}
\def\kg   {\ensuremath{\,\mathrfm{kg}}\xspace}
\def\ton  {\ensuremath{{\,\mathrm{t}}}\xspace}

\def\gmps {\ensuremath{\,\mathrm{g/s}}\xspace} 


%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{{\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\,\mathrm{ms}}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu\mathrm{s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\,\mathrm{ns}}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\,\mathrm{ps}}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\eg{\ensuremath\mathrm{e.g.}}
\def\ie{\ensuremath\mathrm{i.e.}}

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\pct {\ensuremath{{\,\mathrm{\%}}}\xspace}

\def\cms         {\ensuremath{{\,\mathrm{cm}}^{-2} {s}^{-1}}\xspace}

\def\muF  {\ensuremath{\,\mu\mathrm{F}}\xspace}
\def\muH  {\ensuremath{\,\mu\mathrm{H}}\xspace}
\def\nF   {\ensuremath{\,\mathrm{nF}}\xspace}
\def\nH   {\ensuremath{\,\mathrm{nH}}\xspace}
\def\mic  {\ensuremath{\,\mu\mathrm{C}}\xspace}
\def\krad {\ensuremath{\,\mathrm{krad}}\xspace}
\def\cmc  {\ensuremath{{\,\mathrm{cm}}^3}\xspace}
\def\yr   {\ensuremath{\,\mathrm{yr}}\xspace}
\def\hr   {\ensuremath{\,\mathrm{hr}}\xspace}
\def\degc {\ensuremath{^\circ}{\mathrm{C}}\xspace}
\def\degk {\ensuremath {\,\mathrm{K}}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\,\mathrm{mrad}}\xspace}               %% milliradian
\def\rad{\ensuremath{\,\mathrm{rad}}\xspace}
\def\mradhyph{\ensuremath{\mathrm{-mr}}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}
\def\thlf  {\ensuremath{\mathrm{T}_{1/2}}\xspace}

%\renewcommand{\bar}[1]{\overline{#1}}

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}


\def\sx    {\ensuremath{\sigma_x}\xspace}
\def\sy    {\ensuremath{\sigma_y}\xspace}
\def\sz    {\ensuremath{\sigma_z}\xspace}


\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq                {\ensuremath{q^2}\xspace}


% Data processing

\def\bit	{\ensuremath{{\,\text{bit}}}\xspace}
\def\kbit	{\ensuremath{{\,\text{kbit}}}\xspace}
\def\kbitps	{\ensuremath{{\,\text{kbit/s}}}\xspace}
\def\kbitsps	{\kbitps} % no more plural of units - deprecated
\def\kbps	{\kbitps} % for compatibility - deprecated
\def\kbsps	{\kbitsps} % for compatibility - deprecated

\def\kbyte      {\ensuremath{{\,\text{kByte}}}\xspace}
\def\kbytes	{\kbyte}
\def\kbyteps    {\ensuremath{{\,\text{kByte/s}}}\xspace}
\def\kbytesps	{\kbyteps}


\def\mbyte	{\ensuremath{{\,\text{MByte}}}\xspace}
\def\mbytes	{\mbyte}
\def\mbyteps	{\ensuremath{{\,\text{MByte/s}}}\xspace}
\def\mbytesps	{\mbyteps}

\def\mbit	{\ensuremath{{\,\text{Mbit}}}\xspace}
\def\mbits	{\mbit}
\def\mbitps	{\ensuremath{{\,\text{Mbit/s}}}\xspace}
\def\mbitsps	{\mbitps}
\def\mbps	{\mbitps} % for compatibility - deprecated
\def\mbsps	{\mbitsps} % for compatibility - deprecated

\def\gbit	{\ensuremath{{\,\text{Gbit}}}\xspace}
\def\gbits	{\gbit}
\def\gbitps	{\ensuremath{{\,\text{Gbit/s}}}\xspace}
\def\gbitsps	{\gbitps}
\def\gbps	{\gbitps} % for compatibility - deprecated
\def\gbsps	{\gbitsps} % for compatibility - deprecated


\def\gbyte	{\ensuremath{{\,\text{GByte}}}\xspace}
\def\gbytes	{\gbyte}
\def\gbyteps	{\ensuremath{{\,\text{GByte/s}}}\xspace}
\def\gbytesps	{\gbyteps}

\def\tbyte	{\ensuremath{{\,\text{TByte}}}\xspace}
\def\tbytes	{\tbyte}
\def\tbyteps	{\ensuremath{{\,\text{TByte/s}}}\xspace}
\def\tbytesps	{\tbyteps}
\def\tbyteph	{\ensuremath{{\,\text{TByte/h}}}\xspace}
\def\tbytesph   {\tbyteph}
\def\tbytepd	{\ensuremath{{\,\text{TByte/day}}}\xspace}
\def\tbytespd   {\tbytepd}

\def\pbyte	{\ensuremath{{\,\text{PByte}}}\xspace}
\def\pbytepy    {\ensuremath{{\,\text{PByte/yr}}}\xspace}

\def\tbpy       {\ensuremath{{\,\text{TByte/yr}}}\xspace}

\def\khs        {\ensuremath{{\,\text{kHS06}}}\xspace}
\def\mhs	{\ensuremath{{\,\text{MHS06}}}\xspace}

\def\tbpab	{\ensuremath{\tbyte/\invab}}
\def\khspab	{\ensuremath{\khs/\invab}}



\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{\ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

%
% Dark Matter
%
\newcommand{\vesc}{\ensuremath{v_{\text{esc}}}\xspace}
\newcommand{\MWIMP}{\ensuremath{M_{\text{WIMP}}}\xspace}
\newcommand{\Emin}{\ensuremath{E_{\text{min}}}\xspace}
\newcommand{\QBB}{\ensuremath{Q_{\!\Pgb\kern-0.1em\Pgb}}\xspace}

%
% Radioactive Isotopes
%
\newcommand{\IXenat}{\HepIsotope{Xe}{}{nat}\xspace}
\newcommand{\IXemes}{\HepIsotope{Xe}{}{m}\xspace}
\newcommand{\IXeotf}{\HepIsotope{Xe}{}{124}\xspace}
\newcommand{\IXeotF}{\HepIsotope{Xe}{}{125}\xspace}
\newcommand{\IXeots}{\HepIsotope{Xe}{}{126}\xspace}
\newcommand{\IXeotS}{\HepIsotope{Xe}{}{127}\xspace}
\newcommand{\IXeote}{\HepIsotope{Xe}{}{128}\xspace}
\newcommand{\IXeotn}{\HepIsotope{Xe}{}{129}\xspace}
\newcommand{\IXeotnm}{\HepIsotope{Xe}{}{129m}\xspace}
\newcommand{\IXeoTz}{\HepIsotope{Xe}{}{130}\xspace}
\newcommand{\IXeoTo}{\HepIsotope{Xe}{}{131}\xspace}
\newcommand{\IXeoTom}{\HepIsotope{Xe}{}{131m}\xspace}
\newcommand{\IXeoTt}{\HepIsotope{Xe}{}{132}\xspace}
\newcommand{\IXeoTT}{\HepIsotope{Xe}{}{133}\xspace}
\newcommand{\IXeoTf}{\HepIsotope{Xe}{}{134}\xspace}
\newcommand{\IXeoTF}{\HepIsotope{Xe}{}{135}\xspace}
\newcommand{\IXeoTs}{\HepIsotope{Xe}{}{136}\xspace}
\newcommand{\IKrnat}{\HepIsotope{Kr}{}{nat}\xspace}
\newcommand{\IKreF}{\HepIsotope{Kr}{}{85}\xspace}
\newcommand{\IKreTm}{\HepIsotope{Kr}{}{83m}\xspace}
\newcommand{\IKreT}{\HepIsotope{Kr}{}{83}\xspace}
\newcommand{\IRbeT}{\HepIsotope{Rb}{}{83}\xspace}
\newcommand{\IAmtfo}{\HepIsotope{Am}{}{241}\xspace}
\newcommand{\IYee}{\HepIsotope{Y}{}{88}\xspace}
\newcommand{\IRntoe}{\HepIsotope{Rn}{}{218}\xspace}
\newcommand{\IRnton}{\HepIsotope{Rn}{}{219}\xspace}
\newcommand{\IRnttz}{\HepIsotope{Rn}{}{220}\xspace}
\newcommand{\IRnttt}{\HepIsotope{Rn}{}{222}\xspace}
\newcommand{\IHT}{\HepIsotope{H}{}{3}\xspace}
\newcommand{\IHeT}{\HepIsotope{He}{}{3}\xspace}
\newcommand{\IArTS}{\HepIsotope{Ar}{}{37}\xspace}
\newcommand{\IArTn}{\HepIsotope{Ar}{}{39}\xspace}
\newcommand{\IArnat}{\HepIsotope{Ar}{}{nat}\xspace}
\newcommand{\ICsoTs}{\HepIsotope{Cs}{}{136}\xspace}
\newcommand{\ICsoTS}{\HepIsotope{Cs}{}{137}\xspace}
\newcommand{\ICftFt}{\HepIsotope{Cf}{}{252}\xspace}
\newcommand{\ICoFS}{\HepIsotope{Co}{}{57}\xspace}
\newcommand{\ICrFo}{\HepIsotope{Cr}{}{51}\xspace}
\newcommand{\IUtTf}{\HepIsotope{U}{}{234}\xspace}
\newcommand{\IUtTF}{\HepIsotope{U}{}{235}\xspace}
\newcommand{\IUtTe}{\HepIsotope{U}{}{238}\xspace}
\newcommand{\IUtTeE}{\HepIsotope{U}{}{238}$_{\mathrm{e}}$\xspace}
\newcommand{\IUtTeL}{\HepIsotope{U}{}{238}$_{\mathrm{l}}$\xspace}
\newcommand{\IUnat}{\HepIsotope{U}{}{nat}\xspace}
\newcommand{\IPatTo}{\HepIsotope{Pa}{}{231}\xspace}
\newcommand{\IPatTT}{\HepIsotope{Pa}{}{233}\xspace}
\newcommand{\IPatTf}{\HepIsotope{Pa}{}{234}\xspace}
\newcommand{\IPatTfm}{\HepIsotope{Pa}{}{234m}\xspace}
\newcommand{\IThttS}{\HepIsotope{Th}{}{227}\xspace}
\newcommand{\IThtte}{\HepIsotope{Th}{}{228}\xspace}
\newcommand{\IThtTz}{\HepIsotope{Th}{}{230}\xspace}
\newcommand{\IThtTo}{\HepIsotope{Th}{}{231}\xspace}
\newcommand{\IThtTt}{\HepIsotope{Th}{}{232}\xspace}
\newcommand{\IThtTtE}{\HepIsotope{Th}{}{232}$_{\mathrm{e}}$\xspace}
\newcommand{\IThtTtL}{\HepIsotope{Th}{}{232}$_{\mathrm{l}}$\xspace}
\newcommand{\IThtTf}{\HepIsotope{Th}{}{234}\xspace}
\newcommand{\IActtS}{\HepIsotope{Ac}{}{227}\xspace}
\newcommand{\IActte}{\HepIsotope{Ac}{}{228}\xspace}
\newcommand{\IRattT}{\HepIsotope{Ra}{}{223}\xspace}
\newcommand{\IRattf}{\HepIsotope{Ra}{}{224}\xspace}
\newcommand{\IRatts}{\HepIsotope{Ra}{}{226}\xspace}
\newcommand{\IRattS}{\HepIsotope{Ra}{}{227}\xspace}
\newcommand{\IRatte}{\HepIsotope{Ra}{}{228}\xspace}
\newcommand{\IFrttT}{\HepIsotope{Fr}{}{223}\xspace}
\newcommand{\IFrttf}{\HepIsotope{Fr}{}{224}\xspace}
\newcommand{\IAttoF}{\HepIsotope{At}{}{215}\xspace}
\newcommand{\IAttoe}{\HepIsotope{At}{}{218}\xspace}
\newcommand{\IAtton}{\HepIsotope{At}{}{219}\xspace}
\newcommand{\IPotoz}{\HepIsotope{Po}{}{210}\xspace}
\newcommand{\IPotoo}{\HepIsotope{Po}{}{211}\xspace}
\newcommand{\IPotot}{\HepIsotope{Po}{}{212}\xspace}
\newcommand{\IPotof}{\HepIsotope{Po}{}{214}\xspace}
\newcommand{\IPotoF}{\HepIsotope{Po}{}{215}\xspace}
\newcommand{\IPotos}{\HepIsotope{Po}{}{216}\xspace}
\newcommand{\IPotoe}{\HepIsotope{Po}{}{218}\xspace}
\newcommand{\IBitzF}{\HepIsotope{Bi}{}{205}\xspace}
\newcommand{\IBitzs}{\HepIsotope{Bi}{}{206}\xspace}
\newcommand{\IBitoz}{\HepIsotope{Bi}{}{210}\xspace}
\newcommand{\IBitoo}{\HepIsotope{Bi}{}{211}\xspace}
\newcommand{\IBitot}{\HepIsotope{Bi}{}{212}\xspace}
\newcommand{\IBitof}{\HepIsotope{Bi}{}{214}\xspace}
\newcommand{\IBitoF}{\HepIsotope{Bi}{}{215}\xspace}
\newcommand{\IPbtzs}{\HepIsotope{Pb}{}{206}\xspace}
\newcommand{\IPbtzS}{\HepIsotope{Pb}{}{207}\xspace}
\newcommand{\IPbtze}{\HepIsotope{Pb}{}{208}\xspace}
\newcommand{\IPbtoz}{\HepIsotope{Pb}{}{210}\xspace}
\newcommand{\IPbtot}{\HepIsotope{Pb}{}{212}\xspace}
\newcommand{\IPbtof}{\HepIsotope{Pb}{}{214}\xspace}
\newcommand{\ITltzs}{\HepIsotope{Tl}{}{206}\xspace}
\newcommand{\ITltzS}{\HepIsotope{Tl}{}{207}\xspace}
\newcommand{\ITltze}{\HepIsotope{Tl}{}{208}\xspace}
\newcommand{\ITltoz}{\HepIsotope{Tl}{}{210}\xspace}
\newcommand{\IHgtos}{\HepIsotope{Hg}{}{206}\xspace}
\newcommand{\INatt}{\HepIsotope{Na}{}{22}\xspace}
\newcommand{\IKfz}{\HepIsotope{K}{}{40}\xspace}
\newcommand{\IKft}{\HepIsotope{K}{}{42}\xspace}
\newcommand{\IKnat}{\HepIsotope{K}{}{nat}\xspace}
\newcommand{\IScffm}{\HepIsotope{Sc}{}{44,44m}\xspace}
\newcommand{\IScfs}{\HepIsotope{Sc}{}{46}\xspace}
\newcommand{\IScfS}{\HepIsotope{Sc}{}{47}\xspace}
\newcommand{\IScfe}{\HepIsotope{Sc}{}{48}\xspace}
\newcommand{\IBe}{\HepIsotope{B}{}{8}\xspace}
\newcommand{\IBeS}{\HepIsotope{Be}{}{7}\xspace}
\newcommand{\IBen}{\HepIsotope{Be}{}{9}\xspace}
\newcommand{\INoT}{\HepIsotope{N}{}{13}\xspace}
\newcommand{\INof}{\HepIsotope{N}{}{14}\xspace}
\newcommand{\IOoF}{\HepIsotope{O}{}{15}\xspace}
\newcommand{\IFoS}{\HepIsotope{F}{}{17}\xspace}
\newcommand{\Ipp}{\HepIsotope{p}{}{}\HepIsotope{p}{}{}\xspace}
\newcommand{\Ihep}{\HepIsotope{h}{}{}\HepIsotope{e}{}{}\HepIsotope{p}{}{}\xspace}
\newcommand{\Dnuenue}{\hbox{\Pgn\kern-0.3em\Pe\kern-0.3em$\to$\kern-0.1em\Pgn\kern-0.3em\Pe}\xspace}
\newcommand{\ICosz}{\HepIsotope{Co}{}{60}\xspace}
\newcommand{\IGdoFt}{\HepIsotope{Gd}{}{152}\xspace}
\newcommand{\IGdoFF}{\HepIsotope{Gd}{}{155}\xspace}
\newcommand{\IGdoFS}{\HepIsotope{Gd}{}{157}\xspace}
\newcommand{\ICof}{\HepIsotope{C}{}{14}\xspace}
\newcommand{\ILaoTe}{\HepIsotope{La}{}{138}\xspace}
\newcommand{\INptTn}{\HepIsotope{Np}{}{239}\xspace}
\newcommand{\ICsoTf}{\HepIsotope{Cs}{}{134}\xspace}
\newcommand{\IIotF}{\HepIsotope{I}{}{125}\xspace}
\newcommand{\IIotS}{\HepIsotope{I}{}{127}\xspace}
\newcommand{\IIoTo}{\HepIsotope{I}{}{131}\xspace}
\newcommand{\ITeotom}{\HepIsotope{Te}{}{121m}\xspace}
\newcommand{\ITeotTm}{\HepIsotope{Te}{}{123m}\xspace}
%
%  Double Beta Decay
%
%\newcommand{\Pznbb}{\hbox{0\Pgn\kern-4pt\Pgb\kern-4pt\Pgb}}
\newcommand{\Dznbb}{\hbox{0\Pgn\kern-0.35em\Pgb\kern-0.35em\Pgb}\xspace}
\newcommand{\Dtnbb}{\hbox{2\Pgn\kern-0.35em\Pgb\kern-0.35em\Pgb}\xspace}

%
% Chemicals
%
\newcommand{\CNt}{\HepChemical{N}{2}{}\xspace}
\newcommand{\COt}{\HepChemical{O}{2}{}\xspace}
\newcommand{\CHt}{\HepChemical{H}{2}{}\xspace}
\newcommand{\CHf}{\HepChemical{H}{4}{}\xspace}
\newcommand{\CHtO}{\CHt{O}\xspace}
\newcommand{\CClT}{\HepChemical{Cl}{3}{}\xspace}
\newcommand{\CGdClT}{Gd\CClT\xspace}
\newcommand{\CHF}{HF\xspace}
\newcommand{\CHCl}{HCl\xspace}
\newcommand{\CCrt}{\HepChemical{Cr}{2}{}\xspace}
\newcommand{\COT}{\HepChemical{O}{3}{}\xspace}
\newcommand{\CCrtOT}{\CCrt\COT\xspace}
\newcommand{\CHNOT}{HN\COT}
\newcommand{\CAlt}{\HepChemical{Al}{2}{}\xspace}
\newcommand{\CAltOT}{\CAlt\COT\xspace}
\newcommand{\CBaTiOT}{BaTi\COT\xspace}
\newcommand{\CNaI}{NaI\xspace}
\newcommand{\CCHf}{\HepChemical{C}{}{}\CHf\xspace}
%
% Table-related
%
\colorlet{mrocol}{ProcessBlue!100!}
\colorlet{lrocol}{SkyBlue!50!}
\newcommand{\sfbL}{\sffamily\bfseries\Large}
\newcommand{\sfbl}{\sffamily\bfseries\large}
\newcommand{\sfs}{\sffamily\small}
\newcommand{\rmbL}{\rmfamily\bfseries\Large}
\newcommand{\rmbl}{\rmfamily\bfseries\large}
\newcommand{\rms}{\rmfamily\small}
\newcommand{\Tstrut}{\rule{0pt}{2.4ex}}
\newcommand{\Bstrut}{\rule{1ex}{0pt}}
\newcommand{\numlb}[1]{\num[color=Tan]{#1}}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}m{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash}m{#1}}

%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}\xspace}
\def\bbsim      {\mbox{\tt BBsim}\xspace}
\def\beast      {\mbox{\tt Beast}\xspace}
\def\beget      {\mbox{\tt Beget}\xspace}
\def\Bta        {\mbox{\tt Beta}\xspace}
\def\betakfit   {\mbox{\tt BetaKfit}\xspace}
\def\cornelius  {\mbox{\tt Cornelius}\xspace}
\def\evtgen     {\mbox{\tt EvtGen}\xspace}
\def\euclid     {\mbox{\tt Euclid}\xspace}
\def\fitver     {\mbox{\tt FitVer}\xspace}
\def\fluka      {\mbox{\tt Fluka}\xspace}
\def\fortran    {\mbox{\tt Fortran}\xspace}
\def\gcalor     {\mbox{\tt GCalor}\xspace}
\def\geant      {\mbox{\tt GEANT}\xspace}
%\def\geantFour  {\mbox{\tt GEANT4}\xspace}
\def\geantFour  {\mbox{\scshape Geant4}\xspace}
\def\gheisha    {\mbox{\tt Gheisha}\xspace}
\def\hemicosm   {\mbox{\tt HemiCosm}\xspace}
\def\hepevt     {\mbox{\tt{/HepEvt/}}\xspace}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}\xspace}
\def\minuit     {\mbox{\tt Minuit}\xspace}
\def\objegs     {\mbox{\tt Objegs}\xspace}
\def\paw        {\mbox{\tt Paw}\xspace}
\def\Root       {\mbox{\tt Root}\xspace}
\def\squaw      {\mbox{\tt Squaw}\xspace}
\def\stdhep     {\mbox{\tt StdHep}\xspace}
\def\trackerr   {\mbox{\tt TrackErr}\xspace}
\def\turtle     {\mbox{\tt Decay~Turtle}\xspace}
%
%  From Accelerator
%
\def\tenTo#1#2{\ensuremath{10^{#1#2} \cms}\xspace}
\newcommand{\EE}[1] {\ensuremath{\times 10^{#1}}\xspace}
\newcommand{\EEb}[1] {\ensuremath{\times \mathbf{10}^{\mathbf{#1}}}\xspace}
\newcommand{\PM}[2] {\ensuremath{^{+#1}_{-#2}}\xspace}

% Spin Polarization common symbols
\def\ze#1   {\ensuremath{\zeta_{#1}}\xspace}
\newcommand{\VE}[1]  {\ensuremath{\vec{\mathrm{#1}}}\xspace}

% Electrical units
\def\amp    {\ensuremath{{\rm \,\mathrm{A}}}\xspace}
\def\mA     {\ensuremath{{\rm \,\mathrm{mA}}}\xspace}
\def\muA     {\ensuremath{\mu\mathrm{A}}\xspace}
\def\kA	    {\ensuremath{{\,\mathrm{kA}}}\xspace}
\def\nC     {\ensuremath{{\,\mathrm{nC}}}\xspace}
\def\pC     {\ensuremath{{\,\mathrm{pC}}}\xspace}
\def\Ohm    {\ensuremath{{\,\Omega}}\xspace}
\def\mOhm   {\ensuremath{{\,\mathrm{m}\Omega}}\xspace}
\def\kOhm   {\ensuremath{{\,\mathrm{k}\Omega}}\xspace}
\def\MOhm   {\ensuremath{{\,\mathrm{M}\Omega}}\xspace}
\def\V     {\ensuremath{{\,\mathrm{V}}}\xspace}
\def\kV     {\ensuremath{{\,\mathrm{kV}}}\xspace}
\def\MV     {\ensuremath{{\,\mathrm{MV}}}\xspace}
\def\mV     {\ensuremath{{\,\mathrm{mV}}}\xspace}	
\def\Tesla  {\ensuremath{{\,\mathrm{T}}}\xspace}
\def\Gauss  {\ensuremath{{\,\mathrm{G}}}\xspace}
\def\kGauss  {\ensuremath{{\,\mathrm{kG}}}\xspace}
\def\dB     {\ensuremath{{\,\mathrm{dB}}}\xspace}
\def\Henry  {\ensuremath{{\,\mathrm{H}}}\xspace}

% SI energy unit
\def\J      {\ensuremath{{\,\mathrm{J}}}\xspace}
\def\kJ     {\ensuremath{{\,\mathrm{kJ}}}\xspace}
\def\MJ     {\ensuremath{{\,\mathrm{MJ}}}\xspace}

\def\Jpgm   {\ensuremath{{\,\mathrm{J/g}}}\xspace}

% Power
\def\Watt      {\ensuremath{{\,\mathrm{W}}}\xspace}
\def\MW     {\ensuremath{{\,\mathrm{MW}}}\xspace}
\def\kW     {\ensuremath{{\,\mathrm{kW}}}\xspace}


% Frequency
\def\Hz     {\ensuremath{{\rm \,Hz}}\xspace}
\def\MHz    {\ensuremath{{\rm \,MHz}}\xspace}
\def\GHz    {\ensuremath{{\rm \,GHz}}\xspace}
\def\kHz    {\ensuremath{{\rm \,kHz}}\xspace}

% Flux
\def\Hzpmma {\ensuremath{{\rm \,Hz/mm^2}}\xspace}
\def\kHzpmma {\ensuremath{{\rm \,kHz/mm^2}}\xspace}

\def\Hzpcma {\ensuremath{{\rm \,Hz/cm^2}}\xspace}
\def\kHzpcma {\ensuremath{{\rm \,kHz/cm^2}}\xspace}

% Neutron fluence, flux
\def\neqpcma {\ensuremath{{\,{\rm n}_{eq}/{\rm cm^2}}}\xspace}
\def\neqpcmaps  {\ensuremath{{\,{\rm n}_{eq}/{\rm cm^2/s}}}\xspace}
\def\neqpcmapyr  {\ensuremath{{\,{\rm n}_{eq}/{\rm cm^2/yr}}}\xspace}



% Time
\def\msec   {\ensuremath{{\rm \,ms}}\xspace}
\def\nsec   {\ensuremath{{\rm \,ns}}\xspace}

% Pressure
\def\Torr  {\ensuremath{{\rm \,Torr}}\xspace}
\def\nTorr  {\ensuremath{{\rm \,nTorr}}\xspace}
\def\Pa     {\ensuremath{{\rm \,Pa}}\xspace}
\def\MPa    {\ensuremath{{\rm \,MPa}}\xspace}

% Length
\def\picom  {\ensuremath{{\rm \,pm}}\xspace}
\def\km  {\ensuremath{{\rm \,km}}\xspace}

% Area
%(in babarsym) \def\mbarn  {\ensuremath{{\rm \,mbarn}}\xspace}

% Angle
\def\muRad  {\ensuremath{{\, \mu \rm rad}}\xspace}

% Force
\def\N     {\ensuremath{{\rm \,N}}\xspace}
\def\kN    {\ensuremath{{\rm \,kN}}\xspace} 
\def\kNpmm {\ensuremath{{\rm \,kN/mm}}\xspace}


\def\bets  {\ensuremath{{\beta^{\star}}}\xspace}
\def\betxs  {\ensuremath{{\beta_{x}^{\star}}}\xspace}
\def\betys  {\ensuremath{{\beta_{y}^{\star}}}\xspace}

\def\betx   {\ensuremath{{\beta_{x}}}\xspace}
\def\bety   {\ensuremath{{\beta_{y}}}\xspace}


\def\epsx   {\ensuremath{{\varepsilon_{x}}}\xspace}
\def\epsy   {\ensuremath{{\varepsilon_{y}}}\xspace}

\def\xix  {\ensuremath{{\xi_{x}}}\xspace}
\def\xiy  {\ensuremath{{\xi_{y}}}\xspace}

\def\thx  {\ensuremath{{\theta}}\xspace}
\def\piwi {\ensuremath{{\varphi}}\xspace}
\def\CW   {CW\xspace}
\def\br   {\ensuremath{B\rho}\xspace}
\def\thr  {\ensuremath{\theta_{r}}\xspace}

% Note: original symbol Bz conflicts with what is defined in babarsym
\def\Bzed   {\ensuremath{B_{z}}\xspace}

\def\Be   {Be\xspace}
\def\Cu   {Cu\xspace}
\def\Au   {Au\xspace}
\def\CO2  {$\mathrm{CO}_2$\xspace}


\newcommand{\TODO}[1] {{\color{red} \mbox{ #1}}\xspace}


% Note: for Debbie Ceder, 10/8/2015
%\newcommand{\gtwid}{\mathrel{\raise.3ex\hbox{$>$\kern-.75em\lower1ex\hbox{$\sim$}}}}
%\newcommand{\ltwid}{\mathrel{\raise.3ex\hbox{$<$\kern-.75em\lower1ex\hbox{$\sim$}}}}

